Statistical Challenges in Modeling Big Brain Signals

Brain signal data are inherently big: massive in amount, complex in structure, and high in dimensions. These characteristics impose great challenges for statistical inference and learning. Here we review several key challenges, discuss possible solutions, and highlight future research directions.

==> ref.tex <==

@article{prado2013sequential,
	title={Sequential parameter learning and filtering in structured autoregressive state-space models},
	author={Prado, Raquel and Lopes, Hedibert F},
	journal={Statistics and Computing},
	pages={1--15},
	year={2013},
	publisher={Springer}
}
@article{reiss2007functional,
	title={Functional principal component regression and functional partial least squares},
	author={Reiss, Philip T and Ogden, R Todd},
	journal={Journal of the American Statistical Association},
	volume={102},
	number={479},
	pages={984--996},
	year={2007},
	publisher={Taylor \& Francis}
}

@book{deuschl1999recommendations,
	title={Recommendations for the practice of clinical neurophysiology: guidelines of the International Federation of Clinical Neurophysiology},
	author={Deuschl, G{\"u}nther and Eisen, Andrew and others},
	year={1999},
	publisher={Elsevier}
}
@article{redheffer1977completeness,
	title={Completeness of sets of complex exponentials},
	author={Redheffer, Raymond M},
	journal={Advances in Mathematics},
	volume={24},
	number={1},
	pages={1--62},
	year={1977},
	publisher={Elsevier}
}


@article{wang2016exploratory,
	title={Exploratory Analysis of High Dimensional Time Series with Applications to Multichannel Electroencephalograms},
	author={Wang, Yuxiao and Ting, Chee-Ming and Ombao, Hernando},
	journal={arXiv preprint arXiv:1610.07684},
	year={2016}
}







@article{ombao2001automatic,
	title={Automatic statistical analysis of bivariate nonstationary time series},
	author={Ombao, Hernando C and Raz, Jonathan A and von Sachs, Rainer and Malow, Beth A},
	journal={Journal of the American Statistical Association},
	volume={96},
	number={454},
	pages={543--560},
	year={2001},
	publisher={Taylor \& Francis}
}
@article{ombao2002slex,
	title={The SLEX model of a non-stationary random process},
	author={Ombao, Hernando and Raz, Jonathan and von Sachs, Rainer and Guo, Wensheng},
	journal={Annals of the Institute of Statistical Mathematics},
	volume={54},
	number={1},
	pages={171--200},
	year={2002},
	publisher={Springer}
}

@article{allen2016nonspatial,
	title={Nonspatial sequence coding in CA1 neurons},
	author={Allen, Timothy A and Salz, Daniel M and McKenzie, Sam and Fortin, Norbert J},
	journal={The Journal of Neuroscience},
	volume={36},
	number={5},
	pages={1547--1563},
	year={2016},
	publisher={Soc Neuroscience}
}


@article{fiecas2016modeling,
	title={Modeling the evolution of dynamic brain processes during an associative learning experiment},
	author={Fiecas, Mark and Ombao, Hernando},
	journal={Journal of the American Statistical Association},
	volume={111},
	number={516},
	pages={1440--1453},
	year={2016},
	publisher={Taylor \& Francis}
}

@article{plankar2013principle,
	title={The principle of coherence in multi-level brain information processing},
	author={Plankar, Matej and Bre{\v{z}}an, Simon and Jerman, Igor},
	journal={Progress in biophysics and molecular biology},
	volume={111},
	number={1},
	pages={8--29},
	year={2013},
	publisher={Elsevier}
}


@article{makarova2014can,
	title={Can pathway-specific LFPs be obtained in cytoarchitectonically complex structures?},
	author={Makarova, Julia and Ortu{\~n}o, Tania and Korovaichuk, Alejandra and Cudeiro, Javier and Makarov, Valeri A and Rivadulla, Casto and Herreras, Oscar},
	journal={Frontiers in systems neuroscience},
	volume={8},
	pages={66},
	year={2014},
	publisher={Frontiers}
}

@article{mazzoni2012information,
	title={The information content of Local Field Potentials: experiments and models},
	author={Mazzoni, Alberto and Logothetis, Nikos K and Panzeri, Stefano},
	journal={arXiv preprint arXiv:1206.0560},
	year={2012}
}


@article{einevoll2007laminar,
	title={Laminar population analysis: estimating firing rates and evoked synaptic activity from multielectrode recordings in rat barrel cortex},
	author={Einevoll, Gaute T and Pettersen, Klas H and Devor, Anna and Ulbert, Istvan and Halgren, Eric and Dale, Anders M},
	journal={Journal of neurophysiology},
	volume={97},
	number={3},
	pages={2174--2190},
	year={2007},
	publisher={Am Physiological Soc}
}

@inproceedings{brillinger1964frequency,
	title={A frequency approach to the techniques of principal components, factor analysis and canonical variates in the case of stationary time series},
	author={Brillinger, DR},
	booktitle={Invited Paper, Royal Statistical Society Conference, Cardiff Wales.(Available at http://stat-www.berkeley.edu/users/brill/papers.html)},
	year={1964}
}
@article{makarova2011parallel,
	title={Parallel readout of pathway-specific inputs to laminated brain structures},
	author={Makarova, Julia and Ibarz, Jos{\'e} M and Makarov, Valeri A and Benito, Nuria and Herreras, Oscar},
	journal={Frontiers in systems neuroscience},
	volume={5},
	pages={77},
	year={2011},
	publisher={Frontiers}
}

@article{makarov2010disentanglement,
	title={Disentanglement of local field potential sources by independent component analysis},
	author={Makarov, Valeri A and Makarova, Julia and Herreras, Oscar},
	journal={Journal of computational neuroscience},
	volume={29},
	number={3},
	pages={445--457},
	year={2010},
	publisher={Springer}
}

@article{whitmore2016unmasking,
	title={Unmasking local activity within local field potentials (LFPs) by removing distal electrical signals using independent component analysis},
	author={Whitmore, Nathan W and Lin, Shih-Chieh},
	journal={NeuroImage},
	volume={132},
	pages={79--92},
	year={2016},
	publisher={Elsevier}
}

@article{murthy1996synchronization,
	title={Synchronization of neurons during local field potential oscillations in sensorimotor cortex of awake monkeys},
	author={Murthy, Venkatesh N and Fetz, Eberhard E},
	journal={Journal of Neurophysiology},
	volume={76},
	number={6},
	pages={3968--3982},
	year={1996},
	publisher={Am Physiological Soc}
}


@book{mitzdorf1985current,
	title={Current source-density method and application in cat cerebral cortex: investigation of evoked potentials and EEG phenomena},
	author={Mitzdorf, Ulla and others},
	year={1985},
	publisher={American Physiological Society}
}


@article{vorobyov2002blind,
	title={Blind noise reduction for multisensory signals using ICA and subspace filtering, with application to EEG analysis},
	author={Vorobyov, Sergiy and Cichocki, Andrzej},
	journal={Biological Cybernetics},
	volume={86},
	number={4},
	pages={293--303},
	year={2002},
	publisher={Springer}
}

@article{beckmann2004probabilistic,
	title={Probabilistic independent component analysis for functional magnetic resonance imaging},
	author={Beckmann, Christian F and Smith, Stephen M},
	journal={Medical Imaging, IEEE Transactions on},
	volume={23},
	number={2},
	pages={137--152},
	year={2004},
	publisher={IEEE}
}


@phdthesis{jiru2008relationships,
	title={Relationships between spectral peak frequencies of a causal AR (P) process and arguments of roots of the associated ar polynomial},
	author={Jiru, Abera R},
	year={2008},
	school={San Jose State University}
}



@article{schweppe1965evaluation,
	title={Evaluation of likelihood functions for Gaussian signals},
	author={Schweppe, Fred C},
	journal={Information Theory, IEEE Transactions on},
	volume={11},
	number={1},
	pages={61--70},
	year={1965},
	publisher={IEEE}
}

@book{shumway2013time,
	title={Time series analysis and its applications},
	author={Shumway, Robert H and Stoffer, David S},
	year={2013},
	publisher={Springer Science \& Business Media}
}

@book{hamilton1994time,
	title={Time series analysis},
	author={Hamilton, James Douglas},
	volume={2},
	year={1994},
	publisher={Princeton university press Princeton}
}


@article{arun1990balanced,
	title={Balanced approximation of stochastic systems},
	author={Arun, KS and Kung, SY},
	journal={SIAM journal on matrix analysis and applications},
	volume={11},
	number={1},
	pages={42--68},
	year={1990},
	publisher={SIAM}
}

@inproceedings{zhang2011general,
	title={A general linear non-Gaussian state-space model: Identifiability, identification, and applications},
	author={Zhang, Kun and Hyv{\"a}rinen, Aapo},
	booktitle={JMLR Workshop and Conference Proc., Asian Conf. on Machine Learning},
	pages={113--128},
	year={2011}
}


@article{calhoun2009review,
	title={A review of group ICA for fMRI data and ICA for joint inference of imaging, genetic, and ERP data},
	author={Calhoun, Vince D and Liu, Jingyu and Adal{\i}, T{\"u}lay},
	journal={Neuroimage},
	volume={45},
	number={1},
	pages={S163--S172},
	year={2009},
	publisher={Elsevier}
}


@article{bell1995information,
	title={An information-maximization approach to blind separation and blind deconvolution},
	author={Bell, Anthony J and Sejnowski, Terrence J},
	journal={Neural computation},
	volume={7},
	number={6},
	pages={1129--1159},
	year={1995},
	publisher={MIT Press}
}

@inproceedings{pajunen1996nonlinear,
	title={Nonlinear blind source separation by self-organizing maps},
	author={Pajunen, Petteri and Hyv{\"a}rinen, Aapo and Karhunen, Juha},
	booktitle={In Proc. Int. Conf. on Neural Information Processing},
	year={1996},
	organization={Citeseer}
}

@article{comon1994independent,
	title={Independent component analysis, a new concept?},
	author={Comon, Pierre},
	journal={Signal processing},
	volume={36},
	number={3},
	pages={287--314},
	year={1994},
	publisher={Elsevier}
}

@misc{weinstein1996multi,
	title={Multi-channel signal separation using cross-polyspectra},
	author={Weinstein, Ehud and Yellin, Daniel},
	year={1996},
	month=jul # "~23",
	publisher={Google Patents},
	note={US Patent 5,539,832}
}


@book{hyvarinen2004independent,
	title={Independent component analysis},
	author={Hyv{\"a}rinen, Aapo and Karhunen, Juha and Oja, Erkki},
	volume={46},
	year={2004},
	publisher={John Wiley \& Sons}
}

@misc{hyvarinen2001independent,
	title={Independent components analysis},
	author={Hyvarinen, Aapo and Karhunen, Juha and Oja, Erkki},
	year={2001},
	publisher={Wiley, New York}
}

@article{guo2011general,
	title={A general probabilistic model for group independent component analysis and its estimation methods},
	author={Guo, Ying},
	journal={Biometrics},
	volume={67},
	number={4},
	pages={1532--1542},
	year={2011},
	publisher={Wiley Online Library}
}

@book{niedermeyer2005electroencephalography,
	title={Electroencephalography: basic principles, clinical applications, and related fields},
	author={Niedermeyer, Ernst and da Silva, FH Lopes},
	year={2005},
	publisher={Lippincott Williams \& Wilkins}
}

@article{galin1972lateral,
	title={Lateral specialization of cognitive mode: An EEG study},
	author={Galin, David and Ornstein, Robert},
	journal={Psychophysiology},
	volume={9},
	number={4},
	pages={412--418},
	year={1972},
	publisher={Wiley Online Library}
}

@article{linden1996controlled,
	title={A controlled study of the effects of EEG biofeedback on cognition and behavior of children with attention deficit disorder and learning disabilities},
	author={Linden, Michael and Habib, Thomas and Radojevic, Vesna},
	journal={Biofeedback and self-regulation},
	volume={21},
	number={1},
	pages={35--49},
	year={1996},
	publisher={Springer}
}


@article{makeig1996independent,
	title={Independent component analysis of electroencephalographic data},
	author={Makeig, Scott and Bell, Anthony J and Jung, Tzyy-Ping and Sejnowski, Terrence J and others},
	journal={Advances in neural information processing systems},
	pages={145--151},
	year={1996},
	publisher={Morgan Kaufmann Publishers}
}

@article{jung2000removing,
	title={Removing electroencephalographic artifacts by blind source separation},
	author={Jung, Tzyy-Ping and Makeig, Scott and Humphries, Colin and Lee, Te-Won and Mckeown, Martin J and Iragui, Vicente and Sejnowski, Terrence J},
	journal={Psychophysiology},
	volume={37},
	number={02},
	pages={163--178},
	year={2000},
	publisher={Cambridge Univ Press}
}

@article{anemuller2003complex,
	title={Complex independent component analysis of frequency-domain electroencephalographic data},
	author={Anem{\"u}ller, J{\"o}rn and Sejnowski, Terrence J and Makeig, Scott},
	journal={Neural Networks},
	volume={16},
	number={9},
	pages={1311--1323},
	year={2003},
	publisher={Elsevier}
}

@article{eichele2011eegift,
	title={EEGIFT: group independent component analysis for event-related EEG data},
	author={Eichele, Tom and Rachakonda, Srinivas and Brakedal, Brage and Eikeland, Rune and Calhoun, Vince D},
	journal={Computational intelligence and neuroscience},
	volume={2011},
	pages={9},
	year={2011},
	publisher={Hindawi Publishing Corp.}
}

@article{michel1992localization,
	title={Localization of the sources of EEG delta, theta, alpha and beta frequency bands using the FFT dipole approximation},
	author={Michel, CM and Lehmann, D and Henggeler, B and Brandeis, D},
	journal={Electroencephalography and clinical neurophysiology},
	volume={82},
	number={1},
	pages={38--44},
	year={1992},
	publisher={Elsevier}
}
